Reputation Systems for News on Twitter: A Large-Scale Study

Social networks offer a ready channel for fake and misleading news to spread and exert influence. This paper examines the performance of different reputation algorithms when applied to a large and statistically significant portion of the news that are spread via Twitter. Our main result is that simple algorithms based on the identity of the users spreading the news, as well as the words appearing in the titles and descriptions of the linked articles, are able to identify a large portion of fake or misleading news, while incurring only very low (<1%) false positive rates for mainstream websites. We believe that these algorithms can be used as the basis of practical, large-scale systems for indicating to consumers which news sites deserve careful scrutiny and skepticism.

==> introduction-mdipierro.tex <==
The goal of this paper is study different algorithms for automatically flagging potential Fake News posted on social networks. Our focus in on twitter specifically. There are different types of Fake News that circlate on the Internet and they have become more and more difficult to detect. Some of these news are specifically created to be deceiving and look plausible. They are designed to support some popular viewpoit and reinforce the beliefes of specific groups of readers. It is difficult for traditional fact checking to keep up because of the increasing amount of news posted and the speed at which they propagate. We therefore believe there is a need to automate, at least partially, the process of flagging news that are suspicious or of low quality.

We also observed that classification of news items is not always binary. For example we often encoutered news that are, in our opinion, designed to be misleading but they are not per se false. A typical case is when an isolated true event is used to justify a general assertion even if there is no statistical justification for that assertion. For example a newspaper may report of a crime committed by a person of a given minority, ethnicity, or origin and than make the case that a majority, if not all, members of that group are prone to crime. Another and more subtle case is when the news reports about a person making a false statement but not calling out or attempting to verify the statement, instead discussing the consequences of the statement as if it were true. The news itself is not false because it is reporting about a statement that was indeed made but it is clealy designed to mislead the reader into believing the statement is true. On the other opposite of the spectrum, there may be news of scientific or technical nature which are untrue because reported in an oversimplified manner, but that are not designed to deceive, quite the opposite, they are desigend to bring a complex subject to a broad audience.

We therefore believe there is a spectrum of quality of news that ranges from true to false with many shades gray in between. We also believe that there is a specrtun in the crtitical thinking abilities of users of social networks. Most people can be tricked in sharing fake news occasionally but some will try verify the source and some will not. A minority is willing to believe and repost news items even after being told it the information is false, because it reinforces their point of view.

Starting from this consideration we created a reputation system for Twitter users based on the quality of the news they decided to share by re-twitting.

Our system works as follow. First of all we whitelisted a set of internet domains corresponding to major news outlets including cnn.com, nyt.com, foxnews.com, etc. When then called all tweets from these sources or menining these source that contain a valid url. We then called all re-tweets of the original tweets. We also followed all the url redirects and collected the original full news articles referenced in the tweet. We therefore built a database of web pages of news articles, twitter users and links between them. A link represents a tweet or a re-tweet of those articles.














==> previous.tex <==


Castillo et al. [4] showed that automated classifica- tion techniques can be used to detect news topics from conversational topics and assess their credibility based on various Twitter features. They achieved a precision and recall of 70-80\% using a decision-tree based algorithm. Gupta and Kumaraguru [7] in their work on analyzing tweets posted during the terrorist bomb blasts in Mumbai (India, 2011), showed that the majority of sources of information are unknown and have low Twitter reputation (small number of fol- lowers). The authors in a follow up study applied machine learning algorithms (SVM-rank) and information retrieval techniques\
 (relevance feedback) to assess credibility of content on Twitter [8], finding that only 17\% of the total tweets posted about the event contained situational awareness information that was credible. Another, similar work was done by Xia et al. [19] on tweets generated during the England riots of 2011. They used a supervised method based on a Bayesian Network to predict the credibility of tweets in emergency situations. O’Donovan et al. [15] focused their work on finding indicators of credibility during different situations (8 separate event tweets were considered). Their results showed that the best indicators of credibility were URLs, mentions, retweets and tweet length.

[4] Castillo, C., Mendoza, M., Poblete, B.: Information credibility on Twitter. In: Proc. WWW. pp. 675–684. ACM (2011), http://doi.acm.org/10.1145/
1963405.1963500

[7] Gupta, A., Kumaraguru, P.: Twitter explodes with activity in Mumbai blasts! a lifeline or an unmonitored daemon in the lurking? Tech. Rep.
IIITD-TR-2011-005, IIIT, Delhi (2011)

[8] Gupta, A., Kumaraguru, P.: Credibility ranking of tweets during high im-
pact events. In: Proc. 1st Workshop on Privacy and Security in Online Social Media. pp. 2:2–2:8. PSOSM ’12, ACM (2012), http://doi.acm.org/ 10.1145/2185354.2185356

[19] Xia, X., Yang, X., Wu, C., Li, S., Bao, L.: Information credibility on Twitter in emergency situation. In: Proc. Pacific Asia conference on Intelligence and Security Informatics. PAISI’12 (2012)

[15] O’Donovan, J., Kang, B., Meyer, G., Hllerer, T., Adali, S.: Credibility in context: An analysis of feature distributions in Twitter. ASE/IEEE Inter- national Conference on Social Computing, SocialCom (2012)

Thus, various authors agree on the need of auto-
50 matic, computational hoax detection systems [7, 12, 25]. As argued
51 by Ciampaglia et al. [7], this “may signi cantly enhance our ability
52 to evaluate the veracity of dubious information”.
Shu et al. [20] recently classi ed fake news detection methods 65 into two categories - news content models and social context mod- 66 els - based on their main input sources. Methods belonging in the 67  rst category focus on the content of the news, i.e. the body-text, 68 the title, and few additional metadata (when available); here, we re- 69 fer to these methods as content-based methods. Methods belonging 70 in the second category focus on social features and signals, such 71 as the engagement and interaction of users with a given news on 72 social media (e.g. “liking” a news on Facebook, “retweeting” it on 73 Twitter, etc.); here, we refer to these methods as social-based meth- 74 ods. A similar classi cation of methods was previously proposed 75 by Conroy et al. [8], who additionally pointed out that “both [types 76 of methods] typically incorporate machine learning (ML) techniques”. 77 Thus, we focus our review solely on ML methods, although other ap- 78 proaches have been proposed, e.g. based on statistical analyses [14] 79 or knowledge graphs [7, 19, 25].
Content-based methods are the traditional approach, as they 81  nd application in conventional news media and - more in general 82 - in all cases in which no social information is available. Histori- 83 cally, these methods have been used for spam detection in email 84 messages [23] and webpages [18]. In the last years, they have also 85 been applied for fake news detection: Badaskar et al. [3] exploited 86 syntactic and semantic features for classifying between real arti- 87 cles and articles generated by sampling a trigram language model, 88 obtaining a 91.5\% accuracy; Wang [24] used convolutional neural 89 networks with text and additional metadata on a large political fake 90 news dataset; in the context of a recent fake news challenge, Riedel 91 et al. [17] showed that using a relatively simple approach based 92 on term frequency (TF) and term frequency-inverse document fre- 93 quency (TF-IDF) could already o er a good baseline accuracy of 94 88.5\%; Ahmed et al. [1] also recently used TF-IDF and six di erent 95 ML classi ers on a 2000 news dataset, obtaining a 92\% accuracy. 96 The main di culty in applying content-based methods for real- 97 world fake news detection is that these news are “intentionally 98 written to mislead consumers, which makes it nontrivial to detect 99
simply based on news content” [21]. Additionally, Potthast et al. [15] 100 recently showed that they could use the news’ writing style to e ec- 101 tively discriminate hyperpartisan news and satire from mainstream 102 news, but they could not claim “to have solved fake news detection 103 via style analysis alone”. These di culties are probably the reason 104 behind the rather limited use of content-based methods for fake 105 news detection on social media. In fact, on platforms such as SNSs, 106 additional information about social context features is available, 107 which can help identifying fake news with higher accuracies com- 108 pared to content-based approaches, as shown by Castillo et al. [5] 109 for the case of Twitter.
Social-based methods make use of this additional information, 111
and thus constitute a more recent and promising strategy for fake 112
news detection on social media [20]. Example of features which 113
have been used for this purpose are the characteristics of users (e.g.
egistration age, number of followers, etc.) - as proposed by Castillo
118 et al. [6] and Gupta et al. [10] for the case of Twitter - or their opin-
119 ions and viewpoints, exploited by Jin et al. [13] to assess credibility
120 of content in the same SNS. An alternative social-based strategy
121 for fake news detection on social media is based on mapping the
122 di usion pattern of information. The rationale behind this strategy
123 lies in the dynamics of social media sharing and interaction; in fact,
124 according to Del Vicario et al. [9], “users tend to aggregate in commu-
125 nities of interest, which causes reinforcement and fosters con rmation
126 bias, segregation, and polarization”, and “users mostly tend to select
127 and share content according to a speci c narrative and to ignore the
128 rest”. The idea has been  rst proposed and implemented by Tac-
129 chini et al. [22], who showed that Facebook posts can be classi ed
130 with high accuracy as hoaxes or non-hoaxes on the basis of the
131 users who “like” them. They applied two ML algorithms (logistic
132 regression and harmonic boolean label crowdsourcing) using the
133 IDs of users as features to classify posts, and obtained accuracies
134 exceeding 99% even with very small training sets.
135 Although the method proposed by Tacchini et al. [22] o ers di cult-
136 to-beat performance, its application is inherently limited to cases in
137 which information about the propagation of news in the network
138 is available. In other words, as the method uses social interactions
139 (i.e. “likes”) as signals to help classifying Facebook posts, it cannot
140 be used when a post has no likes, and it will presumably perform
141 worse when a post collects only few social interactions. Having
142 little information about social interactions is a rather typical situa-
143 tion on SNSs, e.g. in the case of just-posted content (early detection),
144 or when information is shared through copy-pasting across the
145 network.


[1] ahmed_detection_2017
[2] allcott_social_2017
[3] badaskar_identifying_2008
[4] del_vicario_spreading_2016
[5] castillo_information_2011
[6] castillo_predicting_2013
[7] ciampaglia_computational_2015
[8] conroy_automatic_2015
[9] del_vicario_spreading_2016
[10] gupta_tweetcred:_2014
[11] gupta_2013
[12] hernandez_first_2002
[13] 



